Daily Deals: Prediction, Social Diffusion, and Reputational Ramifications

Daily deal sites have become the latest Internet sensation, providing discounted offers to customers for restaurants, ticketed events, services, and other items. We begin by undertaking a study of the economics of daily deals on the web, based on a dataset we compiled by monitoring Groupon and LivingSocial sales in 20 large cities over several months. We use this dataset to characterize deal purchases; glean insights about operational strategies of these firms; and evaluate customers' sensitivity to factors such as price, deal scheduling, and limited inventory. We then marry our daily deals dataset with additional datasets we compiled from Facebook and Yelp users to study the interplay between social networks and daily deal sites. First, by studying user activity on Facebook while a deal is running, we provide evidence that daily deal sites benefit from significant word-of-mouth effects during sales events, consistent with results predicted by cascade models. Second, we consider the effects of daily deals on the longer-term reputation of merchants, based on their Yelp reviews before and after they run a daily deal. Our analysis shows that while the number of reviews increases significantly due to daily deals, average rating scores from reviewers who mention daily deals are 10% lower than scores of their peers on average.

==> conclusion.tex <==
\section{Conclusion and Future Work}

Our examination of daily deal sites, and particularly Groupon, has used
data-driven analysis to investigate relationships between deal
attributes and deal size beyond simple measures such as the offer price.  
Indeed, the scope of our investigation goes well outside of deal sites, 
to consider Groupon's relationship with the larger electronic commerce 
ecosystem, including Facebook and Yelp.  We believe we expose significant
complexity in understanding behavior in these systems.   In particular,
predicting deal sizes in settings where price, a multiplicity of other 
deal parameters, as well as the potential for social cascades to affect 
the outcome, provides a clear, albeit difficult, challenge.  We also suggest
the mining of publicly accessible Internet data, such as content on review 
sites, to benchmark the success of deal sites for merchants, in terms of 
the effect on their reputation.  Expanding this approach to other data 
sources (such as Twitter or blogs) could yield further insights.

While our focus here has been on data analysis, we believe our work
opens the door to several significant questions in both modeling and
optimizing deal sites and similar electronic commerce systems.



==> related.tex <==
%%\section{Related Work}

\smallskip

\noindent{\bf Related Work on Daily Deals: } To date, there has been little
previous work examining Groupon and LivingSocial specifically. Edelman et al.
consider the benefits and drawbacks of using Groupon from the side of the
merchant, modeling whether the advertising and price discrimination effects
can make such discounts profitable~\cite{Edelman2010To}. Dholakia polls
businesses to determine their experience of providing a deal with
Groupon~\cite{Dholakia2010How}, and Arabshahi examines their business
model~\cite{Arabshahi2010Undressing}. Several works have studied other online
group buying schemes that arose before Groupon, and that utilize substantially
different dynamic pricing schemes \cite{Anand2003Group,Kauffman2001New}. Ye et
al. recently provide a stochastic ``tipping point'' model for sales from daily
deal sites that incorporates social network effects~\cite{Ye2011}. They
provide supporting evidence for their model using a Groupon data set they
collected that is similar to, but less comprehensive, than ours, but they do
not measure social network activity.

